Risk-Awareness in Learning Neural Controllers for Temporal Logic Objectives

In this paper, we consider the problem of synthesizing a controller in the presence of uncertainty such that the resulting closed-loop system satisfies certain hard constraints while optimizing certain (soft) performance objectives. We assume that the hard constraints encoding safety or mission-critical task objectives are expressed using Signal Temporal Logic (STL), while performance is quantified using standard cost functions on system trajectories. In order to prioritize the satisfaction of the hard STL constraints, we utilize the framework of control barrier functions (CBFs) and algorithmically obtain CBFs for STL objectives. We assume that the controllers are modeled using neural networks (NNs) and provide an optimization algorithm to learn the optimal parameters for the NN controller that optimize the performance at a user-specified robustness margin for the safety specifications. We use the formalism of risk measures to evaluate the risk incurred by the trade-off between robustness margin of the system and its performance. We demonstrate the efficacy of our approach on well-known difficult examples for nonlinear control such as a quad-rotor and a unicycle, where the mission objectives for each system include hard timing constraints and safety objectives.

==> sections/Backprop.tex <==
 In this section, we show how the gradient of specific form of the output feedback
 recurrent model proposed in figure \ref{fig:RNN2} can be computed. Note that this
 includes the dynamics model $\dynamics(.,.)$. According to gradient descent algorithm, we should compute this gradient assuming a known set of parameters $(\theta,\ \vars)$. Here we assume a specific starting state $\state_0\in \init$ and attempt to compute, 
 $$
 \frac{\partial \perfobjective_{\state_0}}{\partial \theta},\ \frac{\partial\perfobjective_{\state_0}}{\partial \vars}=0, \frac{\partial\STLobjective_{\state_0}}{\partial \theta},\ \frac{\partial\STLobjective_{\state_0}}{\partial \vars},
 $$
 for the known parameters $ \vars,\ \theta,\ \state_0$.
 
 \begin{figure}% .... check chat
     \centering
     \includegraphics[width=\linewidth]{Back-prop2.PNG}
     \caption{Shows the layers of parameterized policy DNN in the Proposed output feedback recurrent structure. }
     \label{fig:clarification}
 \end{figure}
 In this section we assume a STL specification, described with formulas $\ev, \alw$ and a conjunction between these formulas. Extending this to a general STL specification is also easy and follows the same approach with little adjustments and we neglect them for page limit. Consider the predicate $\phi_{\alw,i}$ contributes in formula $\alw_{[a_i^\alw,\ b_i^\alw]} \phi_{[\alw,i]},\ i=1,2,...,N_\alw$, and the predicate $\phi_{\ev,i}$ contributes in $\ev_{[a_i^\ev,b_i^\ev]} \phi_{\ev,i}$. Based on algorithm \ref{algo:stl2cbf}, we can propose the following set, that contains all the barriers for predicates contributing to the $\softmin(.)$ function to result in CBF, $\STLobjective_{s_0}$.
 $$\scalebox{0.75}{$
 \mathcal{F}=\Bigg\{ \left\{ \left\{b_{\phi_{\alw,i}(s_j,j)}\right\}_{j=a_i^\alw}^{b_i^\alw} \right\}_{i=1}^{N_\alw} ,
\left\{ \bar{\omega}_{\phi_{\ev,i}}=\frac{\sum_{j=a_i^\ev}^{b_i^\ev} \beta_{i,j-a_i^\ev+1}^2 b_{\phi_{\ev,i}}(s_j,j)}{\sum_{j=a_i^\ev}^{b_i^\ev} \beta_{i,j-a_i^\ev+1}^2} \right\}_{i=1}^{N_\ev}  \Bigg\}$}
 $$
 Thus the cardinality of $\mathcal{F}$ is the number of contributing robustnesses to CBF, where,
 $$
 |\mathcal{F}|=N_\ev+\sum_{i=1}^{N_\alw}(b_i^\alw-a_i^\alw+1)
 $$
 and,
 \begin{equation}
     \frac{\partial \STLobjective_{\state_0}}{\partial \lambda}= \frac{2\lambda}{\eta} \left( \frac{\sum_{i=1}^{|\mathcal{F}|} \mathcal{F}_i \exp(-\eta \mathcal{F}_i)}{\sum_{i=1}^{|\mathcal{F}|}  \exp(-\eta \mathcal{F}_i)}- \STLobjective_{\state_0} \right)
 \end{equation}
 and,
 \begin{equation}
 \begin{aligned}
    & \frac{\partial \STLobjective_{\state_0}}{\partial \beta_{i,j_i}}= \frac{\exp{(-\eta \bar{\omega}_{\phi_{F,i}})}}{ \exp(-\eta\STLobjective_{\state_0})} \Bigg( \frac{2\beta_{j_i} b_{\phi_{\ev,i}}(\state_{a_i^\ev+j_i-1},a_i^\ev+j_i-1)}{ \sum_{j_i=1}^{b_i^\ev-a_i^\ev+1}\beta_{j_i}^2} -\\
    & \hspace{1cm}  \frac{ 2\beta_{j_i}\sum_{j_i=1}^{b_i^\ev-a_i^\ev+1} \beta_{j_i}^2 b_{\phi_{\ev,i}}(\state_{a_i^\ev+j_i-1},a_i^\ev+j_i-1)}{ (\sum_{j_i=1}^{b_i^\ev-a_i^\ev+1}\beta_{j_i}^2)^2}\Bigg)
 \end{aligned}
 \end{equation}
 where $i=1,2,...,N_\ev$ and given an index $i$, then $j_i=1,2,..,b_i^\ev-a_i^\ev+1$.
 
 Before we start the derivative computation for $\param$ we first introduce the dictionary of vectors, $\mathbf{x}=\left\{ x^1,x^2,...,x^{\horizon} \right\}$ where $x^\timeid $ is a vector which contains all the barriers for predicates $b_{\phi_{\alw,i}}(\state_\timeid,\timeid)$ if $t \in [a_i^\alw,b_i^\alw]$ over $i=1,2,...,N_\alw$, and also, $\bar{\omega}_{\phi_{\ev,i}}$ if $t \in [a_i^\ev,b_i^\ev]$ over $i=1,2,...,N_\ev$. Let's assume that the time specified barrier for predicate $b_{\phi_{\alw,i}}(\state_\timeid,\timeid)$ are sorted according to their index $i$ on $x^\timeid $ and afterwards barrier for predicate $\bar{\omega}_{\phi_{\ev,i}}$ are sorted below them again according to their indices $i$. We denote the dimension of vector $x^\timeid $ with $\mathbf{dim}(x^\timeid )$.
 
 We illustrate the derivative computation process with respect to $\theta$ in Fig. \ref{fig:clarification}. Each layer, $j=0,1,...,\ell$ is equipped with the layers of activation functions $\Phi_{j+1}:  \mathbb{R}^{n_{j+1}}\to \mathbb{R}^{n_{j+1}}$, $\Phi_{j+1}=[\phi_1(.),\ \phi_2(.),\ ..., \phi_{n_{j+1}}(.)]^\top $, which $\phi(.)$ is the activation function, $z_{j+1}^\timeid \in \mathbb{R}^{n_{j+1}}$ is the activation of the layer $j+1$ at time $\timeid$,and $y_{j+1}^\timeid \in \mathbb{R}^{n_{j+1}}$ is the pre-activation of the layer $j+1$ at time $\timeid$. We define $n_0=n+1$ as the input size of DNN and $n_{j}$ is size of layers where $W_{j}\in \mathbb{R}^{n_{j+1}\times n_j}$ is the weight matrix and  $b_j\in \mathbb{R}^{n_{j+1}}$, is the bias vector. For each Weight matrix $W_j$ we refer to one of its rows by $W_j(m_j,:)$, and one element of vector $b_j$ by $b_j(m_j)$ where $m_j \in \left\{ 1,2,..., n_{j+1}\right\}$. The output of DNN is the action $\action_{\timeid-1}\in \mathbb{R}^m$ therefore define $n_{\ell+2}=m$. We denote the $i$-th main unit vector of Cartesian coordinates by $e_i$, therefore $e_{m_j}$ is the mentioned unit vector with dimension $n_{j+1}$.
 
 Consider the Recurrent structure proposed in Figure \ref{fig:RNN2}, the value function  $\perfobjective_{\state_0}$ is formulated based on states $\left\{ \state_1,\state_2,...,\state_\horizon\right\}$, on the other hand a random perturbation in $W_j(m_j,:)$ generates perturbation on all of these states, this implies,  
 \begin{equation}\label{eq:1}
 \frac{\partial \perfobjective_{\state_0}}{\partial W_j(m_j,:)}=\sum_{\timeid=1}^\horizon \frac{\partial \perfobjective_{\state_0}}{\partial \state_\timeid} \frac{\partial \state_\timeid}{\partial W_j(m_j,:)},\  j=0,...,\ell+1
 \end{equation}
 Furthermore, consider the recurrent structure proposed in Fig. \ref{fig:RNN2}, the STL specification parameter $\STLobjective_{\state_0}$ is also formulated based on states $\left\{ \state_1,\state_2,...,\state_\horizon\right\}$, and a random perturbation in $W_j(m_j,:)$ generates perturbation on all of these states, this also implies, 
 \begin{equation}\label{eq:2}
 \frac{\partial \STLobjective_{\state_0}}{\partial W_j(m_j,:)}=\sum_{\timeid=1}^\horizon \frac{\partial \STLobjective_{\state_0}}{\partial \state_\timeid} \frac{\partial \state_\timeid}{\partial W_j(m_j,:)},\  j=0,...,\ell+1
 \end{equation}
 The same conclusion is also valid for the perturbation on $b_j(m_j)$ which implies,  
 \begin{equation}\label{eq:3}
 \frac{\partial \perfobjective_{\state_0}}{\partial b_j(m_j)}=\sum_{\timeid=1}^\horizon \frac{\partial \perfobjective_{\state_0}}{\partial \state_\timeid} \frac{\partial \state_\timeid}{\partial b_j(m_j)},\  j=0,...,\ell+1
 \end{equation}
 \begin{equation}\label{eq:4}
 \frac{\partial \STLobjective_{\state_0}}{\partial b_j(m_j)}=\sum_{\timeid=1}^\horizon \frac{\partial \STLobjective_{\state_0}}{\partial \state_\timeid} \frac{\partial \state_\timeid}{\partial b_j(m_j)},\  j=0,...,\ell+1
 \end{equation}
 
 Inspired by the idea of back propagation ${\partial \STLobjective_{\state_0}}/{\partial \state_\timeid}$ and  ${\partial \perfobjective_{\state_0}}/{\partial \state_\timeid}$ are computable iteratively, where,  
 \begin{equation}\label{eq:5}
 \frac{\partial \STLobjective_{\state_0}}{\partial \state_\timeid}=\left(\sum_{i_\timeid =1}^{\mathbf{dim(x^\timeid )}}\frac{\partial \STLobjective_{\state_0}}{\partial x^\timeid _{i_\timeid }}\frac{\partial x^\timeid _{i_\timeid }}{\partial \state_\timeid }\right)+\frac{\partial \STLobjective_{\state_0}}{\partial \state_{\timeid+1}}\frac{\partial \state_{\timeid+1}}{\partial \state_\timeid }
 \end{equation}
 and,
 \begin{equation}\label{eq:6}
 \frac{\partial \perfobjective_{\state_0}}{\partial \state_\timeid }=\frac{\partial \perfobjective_{\state_0}}{\partial r(\state_\timeid )}\frac{\partial r(\state_\timeid )}{\partial \state_\timeid }+\frac{\partial \perfobjective_{\state_0}}{\partial \state_{\timeid+1}}\frac{\partial \state_{\timeid+1}}{\partial \state_\timeid }
 \end{equation}
 where due to the inclusion of dynamics model $\dynamics(.,.)$ in the recurrent structure, the derivative for the term ${\partial \state_{\timeid+1}}/{\partial \state_\timeid }$ is different from what is existent in the literature which is provided in equation, \eqref{eq:7}.
 \begin{equation}\label{eq:7}
 \begin{aligned}
 D_\timeid &=\frac{\partial \state_\timeid }{\partial \state_{\timeid-1}}=\underbrace{\frac{\partial \dynamics(\state_{\timeid-1},\action_{\timeid-1})}{\partial \state_{\timeid-1}}}_{\text{computable}, F_{\state,\timeid}}+\\
 &\underbrace{\frac{\partial \dynamics(\state_{\timeid-1},\action_{\timeid-1})}{\partial \action_{\timeid-1}}}_{\text{computable}, F_{\action,\timeid}} W_{\ell+1}\left(\prod_{\timeid=1}^{\ell}\mathbf{diag}\left(\Phi'(y_{\ell+2-\timeid}^\timeid )\right)W_{\ell+1-\timeid}\right)\\
 &\mathbf{diag}\left(\Phi'(y_1^\timeid )\right)W_0(:,1:n)
 \end{aligned}
 \end{equation}
 The barrier for predicate, present at time $\timeid$, $x^\timeid _{i_\timeid },\ i_\timeid =1,2,..,\mathbf{dim}(x^\timeid )$ and also the reward function $r(.)$ are assumed to be given, therefore we denote the computable terms,  ${\partial x^\timeid _{i_\timeid }}/{\partial \state_\timeid }=B_{\timeid,i_\timeid }$ and ${\partial r(\state_\timeid )}/{\partial \state_\timeid }=R_\timeid $ and given the defined equations for $\perfobjective_{\state_0}$, $\STLobjective_{\state_0}$ we have,
 \begin{equation}\label{8}
 \frac{\partial \STLobjective_{\state_0}}{\partial x^\timeid _{i_\timeid }}=\frac{\exp{(-\eta x^\timeid _{i_\timeid })}}{\exp{(-\eta \STLobjective_{\state_0})}}=E_{\timeid,i_\timeid }, \ \ 
 \frac{\partial \perfobjective_{\state_0}}{\partial r(\state_\timeid )}=\gamma^{\horizon-\timeid}
 \end{equation}
 Thus following the backpropagation technique we call, $\tau_\timeid ={\partial \perfobjective_{\state_0}}/{\partial \state_\timeid }$ and $\kappa_\timeid ={\partial \STLobjective_{\state_0}}/{\partial \state_\timeid }$ and we are informed from Fig. \ref{fig:RNN2}, that,
 $$
 \tau_\horizon= R_\horizon,\ \kappa_\horizon=\sum_{i_\timeid =1}^{\mathbf{dim}(x^\timeid )}E_{\horizon,i_\timeid } B_{\horizon,i_\timeid }
 $$
 thus based on \eqref{eq:5}, \eqref{eq:6}, we can present the following iteration to compute for $\kappa_\timeid , \tau_\timeid $, for  $\timeid=1,...,\horizon$.
 \begin{equation}\label{eq:9}
 \begin{aligned}
 &\kappa_\timeid = \left(\sum_{i_\timeid =1}^{\mathbf{dim}(x^\timeid )} E_{\timeid,i_\timeid } B_{\timeid,i_\timeid } \right) + \kappa_{\timeid+1}D_{\timeid+1},\\
 &\tau_\timeid = \gamma^{\horizon-\timeid} R_\timeid  + \tau_{\timeid+1}D_{\timeid+1}
 \end{aligned}
 \end{equation}
 Here we deal with the terms $\partial \state_\timeid / \partial \theta$, we should mention in advance that the inclusion of dynamics model in the recurrent structure requires this term to be computed again in an iterative procedure like $\tau_\timeid ,\kappa_\timeid $ which this iteration is not required for the standard RNN networks in the literature, on the other hand the presence of this dynamics model requires us to separate gradient computation for $j=0,...,\ell$ and $j=\ell+1$,
 
 $j=0,1,...,\ell$:  In this case we define ${\partial \state_\timeid }/{\partial W_j(m_j,:)}=\sigma_{W_j,\timeid}^{m_j}$ and ${\partial \state_\timeid }/{\partial b_j(m_j)}=\sigma_{b_j,\timeid}^{m_j}$ we can formulate $\state_\timeid =\dynamics(\state_{\timeid-1}, DNN_j(z_{j+1}^\timeid ))$ where $DNN_j$ is a portion of controller DNN with input $z_{j+1}^\timeid $ and output $\action_{\timeid-1}$, on the other hand the perturbation on $W_j(m_j,:)$, $b_j(m_j)$ are effective on both parameters $z_{j+1}^\timeid $ and $\state_{\timeid-1}$, therefore we expand $\partial \state_\timeid /\partial \theta$ as,
 \begin{equation}\label{eq:10}
     \begin{aligned}
      &\frac{\partial \state_\timeid }{\partial W_j(m_j,:)}=\frac{\partial \state_\timeid }{\partial z_{j+1}^\timeid }\frac{\partial z_{j+1}^\timeid }{\partial W_j(m_j,:)}+F_{\state,\timeid}\frac{\partial \state_{\timeid-1}}{\partial W_j(m_j,:)}\\
      &\frac{\partial \state_\timeid }{\partial b_j(m_j)}=\frac{\partial \state_\timeid }{\partial z_{j+1}^\timeid }\frac{\partial z_{j+1}^\timeid }{\partial b_j(m_j)}+ F_{\state,\timeid}\frac{\partial \state_{\timeid-1}}{\partial b_j(m_j)}
     \end{aligned}
 \end{equation}
 In addition $V_j^\timeid ={\partial \state_\timeid }/{\partial z_{j+1}^\timeid }$ is readily accessible with chain rule as,
 \begin{equation}
%\label{eq:11}
    V_j^\timeid =F_{\action,\timeid}W_{\ell+1}\prod_{\timeid=1}^{\ell-j}\mathbf{diag}\left(\Phi'(y_{\ell+2-\timeid}^\timeid )\right)W_{\ell+1-\timeid}
 \end{equation}
 on the other hand $z_{j+1}^\timeid =\Phi_{j+1}(W_jz_{j}^\timeid +b_j)$ which implies,
 \begin{equation}
 %\label{eq:11}
    \begin{aligned}
        &\frac{\partial z_{j+1}^\timeid }{\partial W_j(m_j,:)}=e_{m_j} \otimes \phi'(y_{j+1}^\timeid (m_j))z_j^{t\top},\\
        &\frac{\partial z_{j+1}^\timeid }{\partial b_j(m_j)}=e_{m_j} \otimes \phi'(y_{j+1}^\timeid (m_j)) 
    \end{aligned}
 \end{equation}
 Lets call ${\partial \state_\timeid }/{\partial W_j(m_j,:)}=\sigma_{W_j,\timeid}^{m_j}$ and ${\partial \state_\timeid }/{\partial b_j(m_j)}=\sigma_{b_j,\timeid}^{m_j}$, we are also informed $\state_0$ is a constant which implies,
 \begin{equation}\label{eq:12}
 \begin{aligned}
 &\sigma_{W_j,1}^{m_j}=\frac{\partial \state_1}{\partial W_j(m_j,:)}=V_1^j \left( e_{m_j} \otimes \phi'(y_{j+1}^1(m_j))z_j^{1\top} \right)\\
 &\sigma_{b_j,1}^{m_j}=\frac{\partial \state_1}{\partial b_j(m_j,:)}=V_1^j \left( e_{m_j} \otimes \phi'(y_{j+1}^1(m_j)) \right)
 \end{aligned}
 \end{equation}
 because $F_{\state,\timeid}$ is absent for this case. Thus we can introduce the iteration for $\sigma_{W_j,\timeid}^{m_j}$ and $\sigma_{b_j,\timeid}^{m_j}$ as,
 \begin{equation}\label{eq:13}
 \begin{aligned}
 &\sigma_{W_j,\timeid}^{m_j}=V_\timeid ^j \left( e_{m_j} \otimes \phi'(y_{j+1}^\timeid (m_j))z_j^{t\top} \right) + F_\state \sigma_{W_j,\timeid-1}^{m_j}\\
 &\sigma_{b_j,\timeid}^{m_j}=V_\timeid ^j \left( e_{m_j} \otimes \phi'(y_{j+1}^\timeid (m_j)) \right) + F_\state \sigma_{b_j,\timeid-1}^{m_j}
 \end{aligned}
 \end{equation}
 % $$
 % \frac{\partial s_k}{\partial z_{j+1}^k}=\frac{\partial f_d(s_{k-1},a_{k-1})}{\partial a_{k-1}}W_{\ell+1}\prod_{t=1}^{\ell-j}\mathbf{diag}\left(\Phi'(y_{\ell+2-t}^k)\right)W_{\ell+1-t}=V_k^j
 % $$
 
 % $$ 
 % \begin{aligned}
 % &\frac{\partial s_k}{\partial W_j(m_j,:)}}=\sigma_{W_j,k}^{m_j}\\
 % &\frac{\partial s_k}{\partial W_j(m_j,:)}}=\frac{\partial s_k}{\partial z_{j+1}^k}\frac{\partial z_{j+1}^k}{\partial W_j(m_j,:)}+ \underbrace{\frac{\partial f_d(s_{k-1},a_{k-1})}{\partial s_{k-1}}}_{\text{computable} F_s}\frac{\partial s_{k-1}}{\partial W_j(m_j,:)}}
 % \end{aligned}
 % $$
 
 % $$ 
 % \begin{aligned}
 % &\frac{\partial s_k}{\partial b_j(m_j)}}=\sigma_{b_j,k}^{m_j}\\
 % &\frac{\partial s_k}{\partial b_j(m_j)}}=\frac{\partial s_k}{\partial z_{j+1}^k}\frac{\partial z_{j+1}^k}{\partial b_j(m_j)}+ \frac{\partial f_d(s_{k-1},a_{k-1})}{\partial s_{k-1}}\frac{\partial s_{k-1}}{\partial b_j(m_j)}}
 % \end{aligned}
 % $$
 
 
 % $$
 % \begin{aligned}
 % &\frac{\partial z_{j+1}^k}{\partial W_j(m_j,:)}=e_{m_j} \otimes \phi'(y_{j+1}^k(m_j))z_j^{k\top},\\
 % &\frac{\partial z_{j+1}^k}{\partial b_j(m_j)}=e_{m_j} \otimes \phi'(y_{j+1}^k(m_j)) 
 % \end{aligned}
 % $$
 
 % $$
 % \frac{\partial s_1}{\partial W_j(m_j,:)}}=V_1^j \left( e_{m_j} \otimes \phi'(y_{j+1}^1(m_j))z_j^{1\top} \right)=\sigma_{W_j,1}^{m_j}
 % $$
 
 % $$
 % \frac{\partial s_1}{\partial b_j(m_j,:)}}=V_1^j \left( e_{m_j} \otimes \phi'(y_{j+1}^1(m_j)) \right)=\sigma_{b_j,1}^{m_j}
 % $$
 
 % thus,
 % $$
 % \sigma_{W_j,k}^{m_j}=V_k^j \left( e_{m_j} \otimes \phi'(y_{j+1}^k(m_j))z_j^{k\top} \right) + F_s \sigma_{W_j,k-1}^{m_j}
 % $$
 % $$
 % \sigma_{b_j,k}^{m_j}=V_k^j \left( e_{m_j} \otimes \phi'(y_{j+1}^k(m_j)) \right) + F_s \sigma_{b_j,k-1}^{m_j}
 % $$
 
 $j=\ell+1$: We know $\state_\timeid =\dynamics(\state_{\timeid-1},\action_{\timeid-1})$ where $\action_{\timeid-1}=W_{\ell+1}z_{\ell+1}^\timeid +b_{\ell+1}$, therefore,
 \begin{equation}
 %\label{eq:14}
     \begin{aligned}
     &\frac{\partial \state_\timeid }{\partial W_{\ell+1}(m_{\ell+1},:)}=F_{\state,\timeid}\frac{\partial \state_{\timeid-1}}{\partial W_{\ell+1}(m_{\ell+1},:)}+ F_{\action,\timeid}\frac{\partial \action_{\timeid-1}}{\partial W_{\ell+1}(m_{\ell+1},:)}\\
     &\frac{\partial \state_\timeid }{\partial b_{\ell+1}(m_{\ell+1})}=F_{\state,\timeid}\frac{\partial \state_{\timeid-1}}{\partial b_{\ell+1}(m_{\ell+1})}+ F_{\action,\timeid}\frac{\partial \action_{\timeid-1}}{\partial b_{\ell+1}(m_{\ell+1})}
     \end{aligned}
 \end{equation}\label{eq:15}
 We know $\action_{\timeid-1}=W_{\ell+1}z_{\ell+1}^\timeid +b_{\ell+1}$, therefore ,
 \begin{equation}\label{eq:14}
     \frac{\partial \action_{\timeid-1}}{\partial W_{\ell+1}(m_{\ell+1},:)}= e_{m_{\ell+1}} \otimes z_{\ell+1}^{t\top}, \quad \frac{\partial \action_{\timeid-1}}{\partial b_{\ell+1}(m_{\ell+1},:)}= e_{m_{\ell+1}} 
 \end{equation}
 Lets call $\sigma_{W_{\ell+1},\timeid}^{m_{\ell+1}}={\partial \state_\timeid }/{\partial W_{\ell+1}(m_{\ell+1},:)}$, and $\sigma_{b_{\ell+1},\timeid}^{m_{\ell+1}}={\partial \state_\timeid }/{\partial b_{\ell+1}(m_{\ell+1},:)}$. We know $\state_0$ is constant, therefore,
 \begin{equation}
     \sigma_{W_{\ell+1},1}^{m_{\ell+1}}= F_{\action,\timeid} \left(e_{m_{\ell+1}}\otimes z_{\ell+1}^{1\top} \right), \quad \sigma_{b_{\ell+1},1}^{m_{\ell+1}}= F_{\action,\timeid} e_{m_{\ell+1}}
 \end{equation}
 Thus we can introduce the iteration, 
 \begin{equation}\label{eq:16}
 \begin{aligned}
 &\sigma_{W_{\ell+1},\timeid}^{m_{\ell+1}}=F_{\state,\timeid} \sigma_{W_{\ell+1},\timeid-1}^{m_{\ell+1}}+F_{\action,\timeid} \left(e_{m_{\ell+1}}\otimes z_{\ell+1}^{t\top} \right)\\
 &\sigma_{b_{\ell+1},\timeid}^{m_{\ell+1}}=F_{\state,\timeid} \sigma_{b_{\ell+1},\timeid-1}^{m_{\ell+1}}+F_{\action,\timeid} e_{m_{\ell+1}}
 \end{aligned}    
 \end{equation}
 This concludes the computation of \eqref{eq:1}, \eqref{eq:2}, \eqref{eq:3}, \eqref{eq:4}, or in another word, $\partial \perfobjective_{\state_0}/\partial \theta$ and $\partial \STLobjective_{\state_0}/\partial \theta$, given an arbitrary constant $\state_0$.
 
 % Finally given a set of initial conditions, $\mathcal{D}=\left\{ s_0^1,s_0^2,...,s_0^N\right\}$, we compute, 
 % \begin{equation}\label{eq:17}
 % \begin{aligned}
 % &\frac{\partial \mathcal{J}}{\partial \theta}=\sum_{i=1}^N \left(\frac{1}{N}\frac{\partial \mathcal{J}^1_{s_0^i}}{\partial \theta}+ \delta_i^2 \frac{\partial \mathcal{J}^2_{s_0^i}}{\partial \theta} \right) \\
 % &\frac{\partial \mathcal{J}}{\partial \lambda}=\sum_{i=1}^N \delta_i^2 \frac{\partial \mathcal{J}^2_{s_0^i}}{\partial \lambda}, \quad \frac{\partial \mathcal{J}}{\partial \delta_i}= 2 \delta_i \mathcal{J}^2_{s_0^i}
 % \end{aligned}
 % \end{equation}
 
 % $$
 % \frac{\partial s_k}{\partial W_{\ell+1}(m_{\ell+1},:)}=\sigma_{W_{\ell+1},k}^{m_{\ell+1}},
 % $$
 % $$
 % \frac{\partial a_{k-1}}{\partial W_{\ell+1}(m_{\ell+1},:)}= e_{m_{\ell+1}} \otimes z_{\ell+1}^{k\top}
 % $$
 
 % therefore:
 % $$
 % \sigma_{W_{\ell+1},1}^{m_{\ell+1}}= F_a \left(e_{m_{\ell+1}}\otimes z_{\ell+1}^{1\top} \right)
 % $$
 
 % $$
 % \sigma_{W_{\ell+1},k}^{m_{\ell+1}}=F_s \sigma_{W_{\ell+1},k-1}^{m_{\ell+1}}+F_a \left(e_{m_{\ell+1}}\otimes z_{\ell+1}^{k\top} \right)
 % $$}

==> sections/scalability.tex <==
\noindent \textsc{Probabilistic Verification:} 
We sample one million data points from the possible initial states and system disturbance. We obtain the corresponding trajectory and robustness value by executing from the sampled initial conditions. We introduce two commonly used risk measures on such robustness values to verify the system behavior.
`
\subsubsection{Risk Measures}

Now the user provide a target confident level $\beta$, and we calculate the corresponding $VaR$, $CVaR$ as in table \ref{tab:verification}. If the risk measure is positive, it indicates that with $100*\beta$ percent of probability, the robustness value will be higher than the risk value.

\noindent \textsc{Compensation for Scalability:} The proposed RNN structure in Fig \ref{fig:RNN2} may suffer from vanishing and exploding gradients if the time horizon $\horizon$ is high. 
Gradient vanishing and explosion have been observed in some NN training problems involving learning systems with long delays and feedback \cite{bengio1994learning}.  Indeed, closed-loop systems with neural networks typically feature nonlinearities which have a tendency to “squash” derivatives resulting from backpropagation through many layers and/or through multiple copies of the same NN in a sequence of time steps.  Such compression could cause vanishingly small, information impoverished gradients.  Simplistic attempts to increase the tiny gradients by drastically increasing the learning rate in the stochastic gradient method often result in training process instabilities due to difficulties controlling gradients rapidly increasing between training iterations.  Paradoxically, the same NN may exhibit both vanishing and explosive gradients if the training process is not carefully designed.  Stable training process should rely not only on more sophisticated methods beyond gradient descent e.g., adaptive learning rates improving ill-conditioning in the NN, but also on organizing the process itself to reduce the probability of dramatic variability of gradients (destabilizing).  It is easy to see why gradient explosion can occur in a long sequence of the closed-loop system including a neurocontroller if weight copies of the neurocontroller corresponding to different time steps in the sequence are changed all at once.  Early in the training process the weights are likely to result in the terminal state (achieved at the end of the sequence) which is quite far away from the target state, resulting in large errors to be propagated to all copies of the weights.  Such large errors are bound to destabilize the training process.  Various countermeasures have been developed over the past 30 years; see, e.g., \cite{Plumer96},\cite{Prokhorov01},\cite{DRNN01},\cite{HGZ06},\cite{NNtricks12},\cite{Fairbank13}.  For example, it is recommended to start the training process closer to the target state (or having fewer steps in the sequence), gradually moving farther away (extending the sequence) from the target state as the neurocontroller gets more competent at controlling the plant/system while optimizing various terms of the cost function \cite{TruckBU}.  Other remedies against training destabilization include: 1) maintaining different copies of the weights of the neurocontroller corresponding to different time steps in the sequence of forward propagated closed-loop systems while changing only the most recent copy of the NN weights at each training iteration, as opposed to all of the weight copies at once; 2) using less terms of the overall cost function early in the training and gradually adding more terms as the training progresses.

